Enabling Reusable Physical Design Flows with Modular Flow Generators

Achieving high code reuse in physical design flows is challenging but increasingly necessary to build complex systems. Unfortunately, existing approaches based on parameterized Tcl generators support very limited reuse and struggle to preserve reusable code as designers customize flows for specific designs and technologies. We present a vision and framework based on modular flow generators that encapsulates coarse-grain and fine-grain reusable code in modular nodes and assembles them into complete flows. The key feature is a flow consistency and instrumentation layer embedded in Python, which supports mechanisms for rapid and early feedback on inconsistent composition. The approach gradually types the Tcl language and allows both automatic and user-annotated static assertion checks. We evaluate the design flows of successive generations of silicon prototypes designed in TSMC16, TSMC28, TSMC40, SKY130, and IBM180 technologies, showing how our approach can enable significant code reuse in future flows.

==> fig-agile-mock.tex <==
%=========================================================================
% fig-agile-mock
%=========================================================================

\begin{figure}[t]

  \centering
  \includegraphics[width=0.9\columnwidth]{f/agile-mock.pdf}

  \caption{\textbf{Unit Development and Test in mflowgen} --
  %
    Modular nodes can be unit developed in a small mock graph before
    deploying to a project graph. The testing collateral can be reused
    with agile continuous integration tools.
  %
  }

  \label{fig-agile-mock}
%  \vspace{-0.1in}

\end{figure}



==> fig-agile-submodular.tex <==
%=========================================================================
% fig-agile-submodular
%=========================================================================

\begin{figure}[t]

  \centering
  \includegraphics[width=\columnwidth]{f/agile-submodular.pdf}

  \caption{\textbf{Tweaking Existing Nodes in mflowgen} --
  %
    Modular nodes can be designed as script runners to add functionality
    while still reusing existing code.
  %
  }

  \label{fig-agile-submodular}
%  \vspace{-0.1in}

\end{figure}



==> fig-results-operators.tex <==
%=========================================================================
% fig-results-operators
%=========================================================================

\begin{figure*}[t]

  \centering
  \includegraphics[width=0.95\textwidth]{f/results-operators.pdf}

  \caption{\textbf{Operator Area/Energy Characterization in 45nm} --
  %
    The area and energy of combinational operators is shown in an
    open-source 45nm technology. Each dot is a separate design with
    a different operator, format (int/fp), datapath bitwidth, and clock
    target. The plot lines end when the post-place-route design fails to
    meet timing.
  %
  }

  \label{fig-results-operators}
%  \vspace{-0.1in}

\end{figure*}



==> fig-results-power-domains.tex <==
%=========================================================================
% fig-results-power-domains
%=========================================================================

\begin{figure*}[t]

  \centering
  \includegraphics[width=0.95\textwidth]{f/results-power-domains.pdf}

  \caption{\textbf{Assertions for Power Domain Clamping Logic} --
  %
    The tile array in Chip16 includes power-gating logic in the tile array
    interconnect (left), which requires mux logic to be specially
    implemented (middle). We append a design-specific assertion to each
    node in place-and-route to guarantee it never breaks.
  %
  }

  \label{fig-results-power-domains}
%  \vspace{-0.1in}

\end{figure*}



==> fig-results-reuse.tex <==
%=========================================================================
% fig-results-reuse
%=========================================================================

\begin{figure*}[t]

  \centering
  \includegraphics[width=1.0\textwidth]{f/plot-reuse-v2.py.pdf}

  \caption{\textbf{Reuse of Common Library Nodes in DenseAccel16} --
  %
    Plot array shows common library nodes (one per column) used
    across three design graphs in DenseAccel16 (one per row) which represent the
    processing element (PE) tile,  full tile array (512 tiles), and the
    full chip. The x-axis
    is a timeline with 6-month, 3-month, and 0-month marks
    before tapeout. The red line measures reuse (i.e., the percentage of  common library lines of code still in use). The blue line is the percentage of the final node's lines of code that are custom. Abbrev: synth~= synthesis; fplan~= floorplan;
    power~= power strategy; place~\&~route~=place, clock tree synthesis, routing, and postroute optimizations; genlibdb~= generating .lib
    and .db for blocks; 
    drc~= design rule check; lvs~= layout versus schematic.
  %
  }

  \label{fig-results-reuse}
  \vspace{-0.1in}

\end{figure*}




==> fig-system-graph-building.tex <==
%=========================================================================
% fig-system-graph-building
%=========================================================================

\begin{figure}[t]

  \centering
  \includegraphics[width=\columnwidth]{f/system-graph-building.pdf}

  \caption{\textbf{Graph-Building DSL} --
  %
    A Python-based embedded DSL is used to programmatically assemble
    modular nodes into a graph that represents a simple synthesis flow.
    A build system generator (not pictured) consumes the graph and
    generates build rules that shuttle files along the edges between
    modular nodes before executing them.
  %
  }

  \label{fig-system-graph-building}
%  \vspace{-0.1in}

\end{figure}


